AbductionRules: Training Transformers to Explain Unexpected Inputs

Transformers have recently been shown to be capable of reliably performing logical reasoning over facts and rules expressed in natural language, but abductive reasoning - inference to the best explanation of an unexpected observation - has been underexplored despite significant applications to scientific discovery, common-sense reasoning, and model interpretability. We present AbductionRules, a group of natural language datasets designed to train and test generalisable abduction over natural-language knowledge bases. We use these datasets to finetune pretrained Transformers and discuss their performance, finding that our models learned generalisable abductive techniques but also learned to exploit the structure of our data. Finally, we discuss the viability of this approach to abductive reasoning and ways in which it may be improved in future work.

==> acknowledgements.tex <==
% First draft ready
\section*{Acknowledgments}
This research was supported by the University of Auckland Postgraduate Honours / PG Diploma Scholarship.

Thanks to Qiming Bao for development of the PARARULE Plus dataset and permission to freely utilise it.
